MovieCuts: A New Dataset and Benchmark for Cut Type Recognition

Understanding movies and their structural patterns is a crucial task in decoding the craft of video editing. While previous works have developed tools for general analysis, such as detecting characters or recognizing cinematography properties at the shot level, less effort has been devoted to understanding the most basic video edit, the Cut. This paper introduces the Cut type recognition task, which requires modeling multi-modal information. To ignite research in this new task, we construct a large-scale dataset called MovieCuts, which contains 173,967 video clips labeled with ten cut types defined by professionals in the movie industry. We benchmark a set of audio-visual approaches, including some dealing with the problem's multi-modal nature. Our best model achieves 47.7% mAP, which suggests that the task is challenging and that attaining highly accurate Cut type recognition is an open research problem. Advances in automatic Cut-type recognition can unleash new experiences in the video editing industry, such as movie analysis for education, video re-editing, virtual cinematography, machine-assisted trailer generation, machine-assisted video editing, among others. Our data and code are publicly available: https://github.com/PardoAlejo/MovieCuts}{https://github.com/PardoAlejo/MovieCuts.

==> figures/teaser_and_cut-types.tex <==
\begin{figure}[t]
    \begin{subfigure}[t]{0.44\linewidth}
    \raggedleft
        \includegraphics[width=1.0\linewidth]{images/understanding_cuts.pdf}
    \caption{\textbf{Cut Type Recognition Task.} There are several types of cuts within a single scene.
    }
    % \caption{\textbf{Cut Type Recognition Task.}
    % Within a movie scene, most of the shot transitions use the \textit{Straight Cut}, or Cut.}
    % \AP{Done! I increased it as much as I could.}\ali{Nice job with the caption here! explicit enough. The text in the figure is too small (all of it), it's really hard to read at regular zoom. There is still white spaces around so it should be possible to make the text bigger.}}

    %In the visuals, we can see the abrupt change between the camera focusing on one of the two actors.
    % \fch{We need a better teaser. Let's start with the most straightforward examples (e.g. a clear cutting on action). Emphasis Cut is also easy to observe.}
    \label{fig:teaser}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.54\linewidth}
    \begin{center}
        \includegraphics[width=\linewidth]{images/dataset_samples.pdf}
    \end{center}
    \caption{\textbf{MovieCuts Dataset Classes.} Each sample in the dataset is composed of two shots and their audio spectogram. 
    % \AP{DONE, I explicitly said that it is a spectogram}\ali{It is not clear to me what the audio signal represents, what do the colors and axes mean? If this is not a common way to represent audio signals then we should specify what it means.}. 
    }
    \label{fig:dataset}
    \end{subfigure}
    
    \caption{ Figure \ref{fig:teaser} illustrates an example of the cut-type recognition tasks. Figure \ref{fig:dataset} shows an example of each of the classes of MovieCuts.
    }
\end{figure}





% \begin{figure*}[ht!]
%     \centering
%     \begin{subfigure}[t]{0.53\linewidth}
%         \centering
%         \raisebox{1.4em}{\includegraphics[width=0.93\linewidth]{images/performance_breakdown_a.pdf}}
%         \caption{Performance breakdown per attribute and dataset characteristics.}
%          \label{fig:performance-breakdown-a}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.47\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/Relative-improvement.pdf}
%         \caption{Audio-visual improvements per cut type}
%          \label{fig:performance-breakdown-b}
%     \end{subfigure}%
%     \caption{\textbf{Performance breakdown.} Here, we showcase a detailed performance analysis. Figure \ref{fig:performance-breakdown-a} shows the performance breakdown according to attributes of MovieCuts, such as type of sound, subjects, locations, duration per clip, and production year. Figure \ref{fig:performance-breakdown-b} shows the performance gain of the audio-visual model versus the visual-only model. For this analysis, we group the cut classes into visual-driven and audio-visual driven.} 
%     \label{fig:performance-breakdown}
%     \vspace{-15pt}
% \end{figure*}

==> tables/test_results.tex <==
\begin{table}[ht!]
    % \small
	\centering
    % \tabcolsep=0.2cm
    % \renewcommand{\arraystretch}{1.1} % Default value: 1

	\begin{tabular}{ c | c | c}
		Model & \textbf{Sampling} & mAP \\
		\hline
		\hline
		AV + Scaled GB\cite{wang2020makes} & Fixed & \textbf{47.70} \\
		\hline
	\end{tabular}
	\caption{\textbf{Test Set Results}. We show the performance of the best model on the test set. The reported number is $\%$ mAP. 
	}
	\label{table:results_test}
\end{table}

==> tables/window_sampling.tex <==
\begin{table}[ht!]
    % \small
	\centering
    % \tabcolsep=0.2cm
    % \renewcommand{\arraystretch}{1.1} % Default value: 1

	\begin{tabular}{ c | c | c}
		Model & \textbf{Sampling} & mAP \\
		\hline
		\hline
		AV + Scaled GB\cite{wang2020makes} & Uniform & 47.17 \\
		\hline
		AV + Scaled GB\cite{wang2020makes} & Gaussian & 47.44 \\
		\hline
		AV + Scaled GB\cite{wang2020makes} & Fixed & \textbf{47.91} \\
		\hline
	\end{tabular}
	\caption{\textbf{Frame Sampling}. We show different window sampling strategies to feed into the network. 
	}
	\label{table:window_sampling}
\end{table}
